The C-Band All-Sky Survey (C-BASS): Design and capabilities

The C-Band All-Sky Survey (C-BASS) is an all-sky full-polarisation survey at a frequency of 5 GHz, designed to provide complementary data to the all-sky surveys of WMAP and Planck, and future CMB B-mode polarization imaging surveys. The observing frequency has been chosen to provide a signal that is dominated by Galactic synchrotron emission, but suffers little from Faraday rotation, so that the measured polarization directions provide a good template for higher frequency observations, and carry direct information about the Galactic magnetic field. Telescopes in both northern and southern hemispheres with matched optical performance are used to provide all-sky coverage from a ground-based experiment. A continuous-comparison radiometer and a correlation polarimeter on each telescope provide stable imaging properties such that all angular scales from the instrument resolution of 45 arcmin up to full sky are accurately measured. The northern instrument has completed its survey and the southern instrument has started observing. We expect that C-BASS data will significantly improve the component separation analysis of Planck and other CMB data, and will provide important constraints on the properties of anomalous Galactic dust and the Galactic magnetic field.

==> commands.tex <==
\makeatletter
\def\ref@jnl#1{{\rmfamily#1}}% 
\newcommand\aj{\ref@jnl{AJ}}% 
          % Astronomical Journal 
\newcommand\araa{\ref@jnl{ARA\&A}}% 
          % Annual Review of Astron and Astrophys 
\newcommand\apj{\ref@jnl{ApJ}}% 
          % Astrophysical Journal 
\newcommand\apjl{\ref@jnl{ApJ}}% 
          % Astrophysical Journal, Letters 
\newcommand\apjs{\ref@jnl{ApJS}}% 
          % Astrophysical Journal, Supplement 
\newcommand\apss{\ref@jnl{Ap\&SS}}% 
          % Astrophysics and Space Science 
\newcommand\aap{\ref@jnl{A\&A}}% 
          % Astronomy and Astrophysics 
\newcommand\aapr{\ref@jnl{A\&A~Rev.}}% 
          % Astronomy and Astrophysics Reviews 
\newcommand\aaps{\ref@jnl{A\&AS}}% 
          % Astronomy and Astrophysics, Supplement 
\newcommand\baas{\ref@jnl{BAAS}}% 
          % Bulletin of the AAS 
\newcommand\memras{\ref@jnl{MmRAS}}% 
          % Memoirs of the RAS 
\newcommand\mnras{\ref@jnl{MNRAS}}% 
          % Monthly Notices of the RAS 
\newcommand\pasa{\ref@jnl{PASA}}% 
          % Publications of the Astronomical Society of Australia 
\newcommand\pra{\ref@jnl{Phys.~Rev.~A}}% 
          % Physical Review A: General Physics 
\newcommand\prb{\ref@jnl{Phys.~Rev.~B}}% 
          % Physical Review B: Solid State 
\newcommand\prc{\ref@jnl{Phys.~Rev.~C}}% 
          % Physical Review C 
\newcommand\prd{\ref@jnl{Phys.~Rev.~D}}% 
          % Physical Review D 
\newcommand\pre{\ref@jnl{Phys.~Rev.~E}}% 
          % Physical Review E 
\newcommand\prl{\ref@jnl{Phys.~Rev.~Lett.}}% 
          % Physical Review Letters 
\newcommand\pasp{\ref@jnl{PASP}}% 
          % Publications of the ASP 
\newcommand\pasj{\ref@jnl{PASJ}}% 
          % Publications of the ASJ 
\newcommand\ssr{\ref@jnl{Space~Sci.~Rev.}}% 
          % Space Science Reviews 
\newcommand\nat{\ref@jnl{Nature}}% 
          % Nature 
\newcommand\na{\ref@jnl{New Astronomy}}% 
          % New Astronomy
\newcommand\nar{\ref@jnl{New Astronomy Reviews}}% 
          % New Astronomy Reviews
\newcommand\iaucirc{\ref@jnl{IAU~Circ.}}% 
          % IAU Cirulars 
\newcommand\aplett{\ref@jnl{Astrophys.~Lett.}}% 
          % Astrophysics Letters 
\newcommand\apspr{\ref@jnl{Astrophys.~Space~Phys.~Res.}}% 
          % Astrophysics Space Physics Research 
\newcommand\nphysa{\ref@jnl{Nucl.~Phys.~A}}% 
          % Nuclear Physics A 
\newcommand\physrep{\ref@jnl{Phys.~Rep.}}% 
          % Physics Reports 
\newcommand\planss{\ref@jnl{Planet.~Space~Sci.}}% 
          % Planetary Space Science 
\newcommand\procspie{\ref@jnl{Proc.~SPIE}}% 
          % Proceedings of the SPIE 
\newcommand\jcap{\ref@jnl{J.~Cosmology and Astroparticle Phys.}}% 
          % Journal of Cosmology and Astroparticle Physics (JCAP) 
\newcommand\qjras{\ref@jnl{Quart.~Jour.~Roy.~Astr.~Soc.}}% 
          % RAS, Quartely Journal 
\let\astap=\aap 
\let\apjlett=\apjl 
\let\apjsupp=\apjs 

\newcommand{\nm}[1]{\textrm{#1}}
\newcommand{\cb}{C-BASS}
\newcommand{\nt}{$90^{\circ}$}
\newcommand{\dr}{\textrm{d}}
\newcommand{\FF}{\vphantom{\vdots}}
\newcommand{\lan}{\langle}
\newcommand{\ran}{\rangle}
\newcommand{\ITMTT}{IEEE Trans. Microw. Theory Tech.}
\newcommand{\IRMTT}{IRE Trans. Microw. Theory Tech.}
\newcommand{\IMTTS}{IEEE Trans. Microw. Theory Tech. Symp. Digest}
\newcommand{\EL}{Electronics Letters}
\newcommand{\IMOTL}{IEEE Microw. Opt. Techn. Letters}


